Waveform Learning under Phase Noise Impairment for Sub-THz Communications

The large untapped spectrum in sub-THz allows for ultra-high throughput communication to realize many seemingly impossible applications in 6G. Phase noise (PN) is one key hardware impairment, which is accentuated as we increase the frequency and bandwidth. Furthermore, the modest output power of the power amplifier demands limits on peak to average power ratio (PAPR) signal design. In this work, we design a PN-robust, low PAPR single-carrier (SC) waveform by geometrically shaping the constellation and adapting the pulse shaping filter pair under practical PN modeling and adjacent channel leakage ratio (ACLR) constraints for a given excess bandwidth. We optimize the waveforms under conventional and state-of-the-art PN-aware demappers. Moreover, we introduce a neural-network (NN) demapper enhancing transceiver adaptability. We formulate the waveform optimization problem in its augmented Lagrangian form and use a back-propagation-inspired technique to obtain a design that is numerically robust to PN, while adhering to PAPR and ACLR constraints. The results substantiate the efficacy of the method, yielding up to 2.5 dB in the required Eb/N0 under stronger PN along with a PAPR reduction of 0.5 dB. Moreover, PAPR reductions up to 1.2 dB are possible with competitive BLER and SE performance in both low and high PN conditions.

==> 0_notepad.tex <==
1.Sub-THz – an enabling technology for ultra high data rates 

2.Phase noise – one of the key challenges 

3.SC-FDE as the candidate waveform

4.Learning the waveform

5.System Model

6.Problem Formulation

7.Trainable constellation

8.Trainable filter

9.AWGN optimal demapper and Neural Demapper

10.Optimization methodology

11.Evaluation setup

12.Results

13.Discussion, conclusions and outlook

==> 2_RelatedWork.tex <==
\label{2_related_work}
In this section we summarize the related literature for PN-robust constellation designs and waveform learning approaches, which are relevant prior work for the method proposed in this work. An algorithm to select constellation points on a lattice, which minimizes the symbol error probability (SEP) under a Tikhonov PN characterization has been presented in \cite{Foschini}. Most of the prior works consider the residual PN, characterized with a Gaussian process assuming an ideal tracker/estimator, which removes the correlated part of the PN. The article \cite{KrishnanSoftMetrics} investigates the maximum likelihood detection in the presence of strong phase noise. The authors derive soft metrics under the assumptions of Gaussian PN and when the probability density function (PDF) of the phase error is unknown but its central moments are known. The subsequent derivation of the symbol error probability encompasses arbitrary constellations. Further contributions in \cite{KrishnanPNOptimization} introduce two approximate maximum likelihood detectors, predicated on high \DM{signal-to-noise ratio} (SNR) and low PN assumptions. These detectors are harnessed for constellation designs via gradient-based optimization, targeting maximum mutual information and symbol error probability, which shows that optimally designed constellations prove resilience against strong phase noise compared to the conventional constellations. However, the optimization criteria does not account for PAPR. Spiral constellations presented in \cite{Spiral} provided a semi-analytic method for defining the constellation, while employing a detection rule originally proposed in \cite{KrishnanPNOptimization}. Recent works aiming at sub-THz on the optimum demodulation and constellation design are  presented in \cite{CEATLetiOptimumDemodulation, CEALetiDigitalDesign}, which proposed polar-QAM and a method of soft-decision decoding compatible with channel coding based on a detection rule proposed in \cite{KrishnanPNOptimization}. However, as noted in \cite{CEALetiDigitalDesign}, both spiral constellations and the polar-QAM have similar PAPR characteristics and their performance improvements under PN come at a significant deterioration of the PAPR. 

%Since, PN becomes a significant problem in optical communications, recent work based on end-to-end learning targeted at constellation shaping with blind phase search is presented in \cite{KIT_DBPS}.

As previously mentioned, \DM{the investigation in} \cite{WaveformFaycal} tackles end-to-end learning of waveforms under PAPR and ACLR constraints. Leveraging a deep convolutional neural receiver, the study optimizes constellations, bit labeling, and pulse shaping filters for SC waveforms across AWGN and fading channels. Noteworthy gains in data rate are achieved with reduced PAPR and ACLR compared to conventional waveforms. However, it is crucial to note that the pulse shaping filters in this approach are \DM{learned in the frequency-domain, and impulse response is obtained through the inverse Fourier transform, leading to} complex-valued \DM{time-domain filters which are} asymmetrical around the peak, diverging from conventional filters. \DM{In this work, we model the oversampled channel compared to the symbol time channel model in \cite{WaveformFaycal}} and aim to learn the filter directly with the impulse response. Additionally, we consider a SC receiver with conventional processing compared to the deep neural receiver which incurs a high computational cost.

